ARMORY: Fully Automated and Exhaustive Fault Simulation on ARM-M Binaries

Embedded systems are ubiquitous. However, physical access of users and likewise attackers makes them often threatened by fault attacks: a single fault during the computation of a cryptographic primitive can lead to a total loss of system security. This can have serious consequences, e.g., in safetycritical systems, including bodily harm and catastrophic technical failures. However, countermeasures often focus on isolated fault models and high layers of abstraction. This leads to a dangerous sense of security, because exploitable faults that are only visible at machine code level might not be covered by countermeasures. In this work we present ARMORY, a fully automated open source framework for exhaustive fault simulation on binaries of the ubiquitous ARM-M class. It allows engineers and analysts to efficiently scan a binary for potential weaknesses against arbitrary combinations of multi-variate fault injections under a large variety of fault models. Using ARMORY, we demonstrate the power of fully automated fault analysis and the dangerous implications of applying countermeasures without knowledge of physical addresses and offsets. We exemplarily analyze two case studies, which are highly relevant for practice: a DFA on AES (cryptographic) and a secure bootloader (non-cryptographic). Our results show that indeed numerous exploitable faults found by ARMORY which occur in the actual implementations are easily missed in manual inspection. Crucially, most faults are only visible when taking machine code information, i.e., addresses and offsets, into account. Surprisingly, we show that a countermeasure that protects against one type of fault can actually largely increase the vulnerability to other fault models. Our work demonstrates the need for countermeasures that, at least in their evaluation, are not restricted to isolated fault models and consider low-level information [...].

==> large_tables/experiment3_absolute.tex <==
\begin{tabular}{crrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
    \toprule
    Opt. &  \multicolumn{1}{c}{Time} &  \multicolumn{8}{c}{Instruction Fault Models} & \multicolumn{14}{c}{Register Fault Models} & \multicolumn{3}{c}{Total Faults} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-10}  \cmidrule(lr){11-24}  \cmidrule(l){25-27} 
    & &  \multicolumn{4}{c}{Permanent} &  \multicolumn{4}{c}{Transient} &  \multicolumn{4}{c}{Permanent} &  \multicolumn{5}{c}{Until Overwrite} & \multicolumn{5}{c}{Transient}& \multicolumn{1}{c}{Instruction}& \multicolumn{1}{c}{Register}& \multicolumn{1}{c}{Combined} \\
    &       &  \multicolumn{1}{c}{\model{1}} &  \multicolumn{1}{c}{\model{2}} &   \multicolumn{1}{c}{\model{3}} &   \multicolumn{1}{c}{\model{4}} &   \multicolumn{1}{c}{\model{5}} &   \multicolumn{1}{c}{\model{6}} &    \multicolumn{1}{c}{\model{7}} &    \multicolumn{1}{c}{\model{8}} & \multicolumn{1}{c}{\model{11}} & \multicolumn{1}{c}{\model{12}} & \multicolumn{1}{c}{\model{13}} & \multicolumn{1}{c}{\model{14}} &  \multicolumn{1}{c}{\model{15}} &  \multicolumn{1}{c}{\model{16}} &   \multicolumn{1}{c}{\model{17}} &  \multicolumn{1}{c}{\model{18}} &   \multicolumn{1}{c}{\model{19}} &  \multicolumn{1}{c}{\model{20}} &  \multicolumn{1}{c}{\model{21}} &   \multicolumn{1}{c}{\model{22}} &   \multicolumn{1}{c}{\model{23}} &    \multicolumn{1}{c}{\model{24}} &&&  \\ 
    
    \cmidrule(lr){3-6} \cmidrule(lr){7-10}  \cmidrule(lr){11-14}  \cmidrule(lr){15-19}   \cmidrule(l){20-24}
    \midrule
    \multicolumn{24}{c}{Analysis I: Secure Boot} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-19} \cmidrule(lr){20-24} \cmidrule(l){25-27}
    O1 & 10489 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 15 & 1 & 0 & 2 & 1 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 2 & 17 & 8 & 25\\
    O2 & 10742 & 1 & 1 & 0 & 7 & 1 & 0 & 0 & 4 & 1 & 0 & 2 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 2 & 14 & 7 & 21\\
    O3 & 6892 & 1 & 1 & 0 & 8 & 1 & 0 & 0 & 6 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 1 & 17 & 4 & 21\\
    Os & 10825 & 1 & 1 & 0 & 2 & 0 & 0 & 0 & 1 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 5 & 3 & 8\\
    \midrule
    \multicolumn{24}{c}{Analysis III: Secure Boot with Instruction Replacement Countermeasure}\\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-19} \cmidrule(lr){20-24} \cmidrule(l){25-27}
    O1 & 31261 & 0 & 1 & 0 & 8 & 0 & 1 & 0 & 262 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 272 & 2 & 274\\
    O2 & 29328 & 0 & 2 & 0 & 19 & 0 & 1 & 0 & 87 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 109 & 2 & 111\\
    O3 & 19255 & 0 & 3 & 0 & 29 & 0 & 2 & 0 & 369 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 403 & 4 & 407\\
    Os & 33267 & 0 & 3 & 0 & 12 & 0 & 2 & 0 & 213 & 1 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 230 & 3 & 233\\
    \midrule
    \multicolumn{24}{c}{Analysis III: Secure Boot with Control Flow Checking Countermeasure}\\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-19} \cmidrule(lr){20-24} \cmidrule(l){25-27}
    O1 & 22258 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 2\\
    O2 & 29476 & 0 & 0 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 3 & 2 & 5\\
    O3 & 10155 & 0 & 0 & 0 & 3 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 3 & 2 & 5\\
    Os & 21737 & 1 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 2 & 4\\
    \midrule
    \multicolumn{24}{c}{Analysis III: Secure Boot with both Countermeasures}\\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-19} \cmidrule(lr){20-24} \cmidrule(l){25-27}
    O1 & 58245 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 2\\
    O2 & 74632 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 2\\
    O3 & 27615 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 2\\
    Os & 57313 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 2\\
    \midrule
    \midrule
    \multicolumn{24}{c}{Analysis I: AES-DFA} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-19} \cmidrule(lr){20-24} \cmidrule(l){25-27}
    O1 & 1320 & 24 & 15 & 25 & 282 & 568 & 136 & 948 & 8082 & 0 & 0 & 0 & 0 & 610 & 636 & 812 & 648 & 7452 & 621 & 717 & 2090 & 943 & 18010 & 10080 & 32539 & 42619\\
    O2 & 1311 & 24 & 24 & 24 & 215 & 566 & 138 & 959 & 6990 & 0 & 0 & 1 & 0 & 570 & 619 & 705 & 608 & 6656 & 633 & 729 & 2112 & 922 & 17990 & 8940 & 31545 & 40485\\
    O3 & 874 & 73 & 31 & 120 & 913 & 503 & 116 & 971 & 6296 & 0 & 0 & 1 & 40 & 568 & 597 & 751 & 618 & 8899 & 533 & 559 & 1279 & 695 & 12887 & 9023 & 27427 & 36450\\
    Os & 1382 & 24 & 16 & 24 & 240 & 590 & 163 & 1096 & 7908 & 0 & 0 & 0 & 0 & 610 & 636 & 908 & 678 & 7997 & 629 & 724 & 2298 & 938 & 18283 & 10061 & 33701 & 43762\\
    \midrule
    \multicolumn{24}{c}{Analysis III: AES-DFA with Instruction Replacement Countermeasure} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-19} \cmidrule(lr){20-24} \cmidrule(l){25-27}
    O1 & 3848 & 0 & 20 & 26 & 316 & 0 & 399 & 1412 & 11060 & 0 & 0 & 0 & 0 & 1658 & 1766 & 2265 & 1880 & 20850 & 877 & 931 & 1372 & 1260 & 13460 & 13233 & 46319 & 59552\\
    O2 & 3877 & 0 & 20 & 54 & 305 & 0 & 429 & 1554 & 11014 & 0 & 0 & 1 & 0 & 1578 & 1732 & 2398 & 1862 & 20953 & 889 & 943 & 1333 & 1256 & 13277 & 13376 & 46222 & 59598\\
    O3 & 2291 & 0 & 24 & 166 & 1147 & 0 & 240 & 1446 & 11146 & 0 & 0 & 0 & 38 & 1517 & 1605 & 2144 & 1631 & 24139 & 725 & 788 & 981 & 902 & 10484 & 14169 & 44954 & 59123\\
    Os & 4007 & 0 & 1 & 26 & 320 & 0 & 375 & 1526 & 10599 & 0 & 0 & 0 & 0 & 1690 & 1798 & 2347 & 1970 & 22560 & 893 & 947 & 1407 & 1276 & 13627 & 12847 & 48515 & 61362\\
    \midrule
    \multicolumn{24}{c}{Analysis III: AES-DFA with Control Flow Checking Countermeasure} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-19} \cmidrule(lr){20-24} \cmidrule(l){25-27}
    O1 & 3074 & 24 & 36 & 64 & 497 & 572 & 275 & 1217 & 9185 & 0 & 0 & 0 & 0 & 610 & 636 & 894 & 680 & 8156 & 621 & 717 & 2079 & 934 & 18114 & 11870 & 33441 & 45311\\
    O2 & 3054 & 24 & 36 & 61 & 477 & 567 & 139 & 1227 & 8187 & 0 & 0 & 0 & 1 & 570 & 618 & 812 & 642 & 7383 & 633 & 729 & 2112 & 928 & 17898 & 10718 & 32326 & 43044\\
    O3 & 1060 & 79 & 40 & 118 & 983 & 614 & 130 & 1203 & 7438 & 0 & 0 & 9 & 43 & 596 & 635 & 831 & 618 & 9597 & 569 & 591 & 1419 & 754 & 14177 & 10605 & 29839 & 40444\\
    Os & 3114 & 24 & 0 & 25 & 191 & 628 & 117 & 1152 & 8321 & 0 & 0 & 0 & 0 & 624 & 653 & 902 & 692 & 8647 & 639 & 731 & 2192 & 930 & 19097 & 10458 & 35107 & 45565\\
    \midrule
    \multicolumn{24}{c}{Analysis III: AES-DFA with both Countermeasures} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-19} \cmidrule(lr){20-24} \cmidrule(l){25-27}
    O1 & 7963 & 0 & 12 & 50 & 394 & 0 & 390 & 1316 & 11522 & 0 & 0 & 0 & 0 & 1658 & 1766 & 2449 & 1942 & 22222 & 877 & 931 & 1361 & 1260 & 13460 & 13684 & 47926 & 61610\\
    O2 & 7899 & 0 & 12 & 50 & 419 & 0 & 367 & 1516 & 10903 & 0 & 0 & 0 & 1 & 1578 & 1730 & 2568 & 1866 & 21105 & 889 & 942 & 1353 & 1256 & 13293 & 13267 & 46581 & 59848\\
    O3 & 2638 & 0 & 32 & 172 & 1212 & 0 & 241 & 1992 & 11189 & 0 & 0 & 9 & 48 & 1543 & 1661 & 2344 & 1587 & 24618 & 739 & 811 & 1024 & 916 & 10769 & 14838 & 46069 & 60907\\
    Os & 8073 & 0 & 0 & 25 & 258 & 0 & 400 & 1497 & 10952 & 0 & 0 & 0 & 0 & 1714 & 1832 & 2657 & 1994 & 23522 & 907 & 963 & 1437 & 1290 & 13868 & 13132 & 50184 & 63316\\
    \bottomrule
\end{tabular}

==> large_tables/experiment4_absolute.tex <==
\begin{tabular}{crrrrrrrrrrrrrrrrrrrrrr}
    \toprule
    Opt. &  \multicolumn{1}{c}{Time} &  \multicolumn{6}{c}{Instruction Fault Models} & \multicolumn{12}{c}{Register Fault Models} & \multicolumn{3}{c}{Total Faults} \\ 
    & &  \multicolumn{3}{c}{2$\times$ Permanent} &  \multicolumn{3}{c}{2$\times$ Transient} &  \multicolumn{4}{c}{2$\times$ Permanent} &  \multicolumn{4}{c}{2$\times$ Until Overwrite} & \multicolumn{4}{c}{2$\times$ Transient}& \multicolumn{1}{c}{Instruction}& \multicolumn{1}{c}{Register}& \multicolumn{1}{c}{Combined} \\
    &       &  \multicolumn{1}{c}{\model{1}} &  \multicolumn{1}{c}{\model{2}} &   \multicolumn{1}{c}{\model{3}} &   \multicolumn{1}{c}{\model{5}} &   \multicolumn{1}{c}{\model{6}} &    \multicolumn{1}{c}{\model{7}} &    \multicolumn{1}{c}{\model{9}}  &    \multicolumn{1}{c}{\model{10}} & \multicolumn{1}{c}{\model{11}} & \multicolumn{1}{c}{\model{12}} & \multicolumn{1}{c}{\model{15}} &  \multicolumn{1}{c}{\model{16}} &   \multicolumn{1}{c}{\model{17}} &  \multicolumn{1}{c}{\model{18}} &    \multicolumn{1}{c}{\model{20}} &  \multicolumn{1}{c}{\model{21}} &   \multicolumn{1}{c}{\model{22}} &   \multicolumn{1}{c}{\model{23}}  &&&  \\ 
    
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}  \cmidrule(lr){9-12}  \cmidrule(lr){13-16}   \cmidrule(l){17-20}
    \midrule
    \multicolumn{23}{c}{Secure Boot} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8}  \cmidrule(lr){9-12}  \cmidrule(lr){13-16}   \cmidrule(lr){17-20} \cmidrule(l){21-23}
    O1 & 10489 & 4 & 6 & 0 & 0 & 0 & 3 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 13 & 1 & 14\\
    O2 & 10742 & 3 & 3 & 3 & 2283 & 10 & 75 & 0 & 0 & 1 & 1 & 0 & 0 & 163 & 0 & 29 & 0 & 505 & 139 & 2377 & 838 & 3215\\
    O3 & 6892 & 3 & 4 & 4 & 457 & 13 & 60 & 1 & 0 & 1 & 4 & 0 & 0 & 137 & 0 & 24 & 0 & 373 & 118 & 541 & 658 & 1199\\
    Os & 10825 & 3 & 2 & 6 & 24 & 16 & 71 & 0 & 0 & 1 & 1 & 0 & 0 & 169 & 0 & 0 & 0 & 177 & 0 & 122 & 348 & 470\\
    \midrule
    \midrule
    \multicolumn{23}{c}{AES-DFA} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8}  \cmidrule(lr){9-12}  \cmidrule(lr){13-16}   \cmidrule(lr){17-20} \cmidrule(l){21-23}
    O1 & 1320 & 24 & 15 & 25 & 1359 & 1776 & 4657 & 0 & 0 & 0 & 0 & 1026 & 4609 & 8432 & 4180 & 1078 & 741 & 8787 & 2549 & 7856 & 31402 & 39258\\
    O2 & 1311 & 24 & 24 & 24 & 640 & 2725 & 5476 & 0 & 0 & 0 & 0 & 859 & 5281 & 17451 & 3632 & 956 & 737 & 8094 & 2279 & 8913 & 39289 & 48202\\
    O3 & 874 & 441 & 176 & 1158 & 509 & 116 & 4463 & 0 & 0 & 0 & 0 & 739 & 598 & 2617 & 815 & 694 & 560 & 4824 & 903 & 6863 & 11750 & 18613\\
    Os & 1382 & 24 & 16 & 24 & 694 & 942 & 9853 & 0 & 0 & 0 & 0 & 1112 & 5264 & 11946 & 4269 & 1169 & 730 & 7937 & 2627 & 11553 & 35054 & 46607\\
    \midrule
    \multicolumn{23}{c}{AES-DFA with Instruction Replacement Countermeasure} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8}  \cmidrule(lr){9-12}  \cmidrule(lr){13-16}   \cmidrule(lr){17-20} \cmidrule(l){21-23}
    O1 & 3848 & 24 & 20 & 36 & 908 & 84435 & 208924 & 0 & 0 & 0 & 0 & 2678 & 24782 & 22168 & 27642 & 1416 & 1034 & 67151 & 4137 & 294347 & 151008 & 445355\\
    O2 & 3877 & 24 & 22 & 60 & 902 & 82430 & 264166 & 0 & 0 & 0 & 0 & 2358 & 23634 & 15480 & 31229 & 2688 & 1024 & 63837 & 6335 & 347604 & 146585 & 494189\\
    O3 & 2291 & 91 & 103 & 3541 & 724 & 22032 & 154830 & 0 & 0 & 0 & 0 & 1845 & 1605 & 8920 & 2027 & 878 & 789 & 4924 & 1101 & 181321 & 22089 & 203410\\
    Os & 4007 & 24 & 1 & 102 & 931 & 75095 & 196033 & 0 & 0 & 0 & 0 & 2281 & 22234 & 15167 & 29202 & 2223 & 1017 & 65319 & 6193 & 272186 & 143636 & 415822\\
    \midrule
    \multicolumn{23}{c}{AES-DFA with Control Flow Checking Countermeasure} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8}  \cmidrule(lr){9-12}  \cmidrule(lr){13-16}   \cmidrule(lr){17-20} \cmidrule(l){21-23}
    O1 & 3074 & 24 & 36 & 69 & 672 & 1209 & 77195 & 0 & 0 & 0 & 0 & 1069 & 5408 & 15403 & 5137 & 1142 & 741 & 10769 & 2754 & 79205 & 42423 & 121628\\
    O2 & 3054 & 24 & 36 & 71 & 644 & 717 & 71223 & 0 & 0 & 0 & 0 & 880 & 5769 & 20821 & 4254 & 981 & 737 & 8281 & 2537 & 72715 & 44260 & 116975\\
    O3 & 1060 & 383 & 97 & 1557 & 620 & 130 & 17881 & 0 & 0 & 0 & 0 & 770 & 635 & 2826 & 826 & 762 & 591 & 5531 & 989 & 20668 & 12930 & 33598\\
    Os & 3114 & 24 & 0 & 25 & 1080 & 614 & 69890 & 0 & 0 & 0 & 0 & 956 & 5058 & 14786 & 5307 & 1378 & 1111 & 15191 & 3697 & 71633 & 47484 & 119117\\
    \midrule
    \multicolumn{23}{c}{AES-DFA with both Countermeasures} \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8}  \cmidrule(lr){9-12}  \cmidrule(lr){13-16}   \cmidrule(lr){17-20} \cmidrule(l){21-23}
    O1 & 7963 & 24 & 48 & 415 & 894 & 143994 & 680678 & 0 & 0 & 0 & 0 & 2841 & 24758 & 31033 & 25382 & 1531 & 1034 & 66745 & 4085 & 826053 & 157409 & 983462\\
    O2 & 7899 & 24 & 48 & 330 & 891 & 118928 & 804341 & 0 & 0 & 0 & 0 & 2408 & 24568 & 19784 & 21946 & 2719 & 1023 & 64577 & 5981 & 924562 & 143006 & 1067568\\
    O3 & 2638 & 98 & 136 & 2682 & 804 & 20430 & 279252 & 0 & 0 & 0 & 0 & 1965 & 1661 & 9841 & 2077 & 960 & 811 & 5201 & 1183 & 303402 & 23699 & 327101\\
    Os & 8073 & 24 & 0 & 43 & 963 & 143689 & 613448 & 0 & 0 & 0 & 0 & 2594 & 24358 & 18995 & 29352 & 2435 & 1034 & 66864 & 6587 & 758167 & 152219 & 910386\\
    \bottomrule
\end{tabular}

==> large_tables/experiment5.tex <==
\begin{tabular}{ccrrr}
   	\toprule
   	Opt. & Fault Model & \multicolumn{2}{c}{\emu} &                $\pm$ \\
	     &             & Generic &       Profiled &                      \\ \midrule
	               \multicolumn{5}{c}{No Countermeasure}                 \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5} \arrayrulecolor{lightgray}
  	 O1  & byte clear  &    1116 &           1116 & \textcolor{gray}{+0} \\
	     &  bit flip   &    9654 &           9686 &                   +2 \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 O2  & byte clear  &    1199 &           1199 & \textcolor{gray}{+0} \\
	     &  bit flip   &    8497 &           8553 &                   +6 \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 O3  & byte clear  &    1053 &           1053 & \textcolor{gray}{+0} \\
	     &  bit flip   &    6962 &           6962 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 Os  & byte clear  &    1297 &           1329 &                  +32 \\
	     &  bit flip   &    9305 &           9305 & \textcolor{gray}{+0} \\ \arrayrulecolor{black} \midrule
	          \multicolumn{5}{c}{Countermeasure: Replacement}            \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5} \arrayrulecolor{lightgray}
  	 O1  & byte clear  &    1589 &           1589 & \textcolor{gray}{+0} \\
	     &  bit flip   &   12838 &          12838 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 O2  & byte clear  &    1835 &           1835 & \textcolor{gray}{+0} \\
	     &  bit flip   &   12908 &          12908 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 O3  & byte clear  &    1587 &           1587 & \textcolor{gray}{+0} \\
	     &  bit flip   &   11936 &          11936 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 Os  & byte clear  &    1780 &           1780 & \textcolor{gray}{+0} \\
	     &  bit flip   &   12426 &          12426 & \textcolor{gray}{+0} \\ \arrayrulecolor{black} \midrule
	          \multicolumn{5}{c}{Countermeasure: Control Flow}           \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5} \arrayrulecolor{lightgray}
  	 O1  & byte clear  &    1440 &           1440 & \textcolor{gray}{+0} \\
	     &  bit flip   &   10984 &          10984 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 O2  & byte clear  &    1483 &           1483 & \textcolor{gray}{+0} \\
	     &  bit flip   &    9856 &           9856 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 O3  & byte clear  &    1287 &           1287 & \textcolor{gray}{+0} \\
	     &  bit flip   &    8164 &           8164 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 Os  & byte clear  &    1345 &           1377 &                  +22 \\
	     &  bit flip   &    9840 &           9840 & \textcolor{gray}{+0} \\\arrayrulecolor{black} \midrule
	              \multicolumn{5}{c}{Countermeasure: Both}               \\ \cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5} \arrayrulecolor{lightgray}
  	 O1  & byte clear  &    1479 &           1479 & \textcolor{gray}{+0} \\
	     &  bit flip   &   13368 &          13368 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 O2  & byte clear  &    1742 &           1742 & \textcolor{gray}{+0} \\
	     &  bit flip   &   12773 &          12773 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 O3  & byte clear  &    2136 &           2136 & \textcolor{gray}{+0} \\
	     &  bit flip   &   12018 &          12018 & \textcolor{gray}{+0} \\\cmidrule(r){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5}
  	 Os  & byte clear  &    1718 &           1718 & \textcolor{gray}{+0} \\
	     &  bit flip   &   12768 &          12768 & \textcolor{gray}{+0} \\ \arrayrulecolor{black} \bottomrule
\end{tabular}

==> sections/revision_report.tex <==
%!TEX root = ../main.tex

\thispagestyle{empty}
\onecolumn

\centerline{\huge{Revision Report}}\ \\
\noindent
This revision report documents our improvements made to the initial submission based on the reviewers' comments.
We sincerely thank all three reviewers for their valuable feedback and the time they invested in reviewing.
To save you time when reading our revision comments, we will not start all our responses with ``thank you'', but rest assured that we truly appreciate your input.
All related changes to the original document, aside from typos and minor fixes, are marked in \revise{blue}.\\

To sum up the major changes in this revision, we adjusted our terminology to be less misleading and heavily rewrote \Section{fsim::sec::armory}, enhancing it with a dedicated section on terminology and another section regarding implications of applying \fsim in real-world applications.
The majority of our presentation of \fsim was restructured to concisely describe its features and output guarantees.
We also adjusted our wording at several points of the paper for improved clarity and expanded our explanations of experiments where necessary.
In total, we are convinced that the reviewer comments resulted in a revision that is more comprehensible for readers of all backgrounds.

\subsection*{Responses to Reviewer Comments}
\thispagestyle{empty}
\subsubsection*{Reviewer 1}
\begin{enumerate}
    \item \textit{Evaluation of whether such faults are exploitable or not is done by a user-set "evaluator function". This implies that the user needs to be aware of the security boundaries of the implemented solution to be able to write such function. It also means that ARMORY can only check the pre-defined vulnerability, but cannot analyze new vulnerabilities. However, I believe this is a hard task when focusing on general solution. There should be a part discussing this, as without a proper evaluation function written by a security expert, vulnerabilities might not be found.}\\
    
        %\todo{OK, allgemeines Problem, ALAFA kann in armory integriert werden, ABER: Ja, AES z.T. eventuell komplizierte Modelle, aber auch einfach „fehlerhafter ciphertext“ oder „kritische Stelle angesprungen unerlaubt“}\\
        \revise{
        We fully agree.
        As in all works on fault assessment, one needs to define a condition which indicates exploitability.
        This can range from simple conditions such as ``an incorrect output is observed'', over more specific models such as ``critical function has been executed'', to highly specialized models as the checks we performed for the AES-DFA explained in \Section{fsim::sec::casestudies::aes}.
        However, all such models are supported out-of-the-box in \fsim.
        }
        
        \revise{
        We updated the terminology in our paper and our explanations in \Section{fsim::sec::armory::inputs} to better capture this notion.
        We also discuss the issue in-depth in our newly added \Section{fsim::sec::armory::realworld} on the implications of applying \fsim in real-world scenarios.
        }\\
    
    \item \textit{Approach described in [A] is related to the proposed method. It should be discussed in Section II.}\\
    
	\revise{We added the following paragraph to Section II.:\\}
    
    \revise{The authors of \cite{DBLP:conf/trustcom/Given-WilsonJLL17} use bounded model checking to automatically verify whether tailored assertions also hold on a modified binary. To this end, the assertions are added in the source code to be compiled alongside. The binary is then modified according to the fault model. Both the genuine and the faulty binary are transferred back to LLVM-IR to be able to check whether the assertions hold. Unfortunately, this approach has some large performance penalty (2 hours for verifying single-bit opcode faults for code that checks a PIN in a loop). Further, formulating assertions on source level that should also cover possible vulnerabilities on assembly level is hard and error-prone.\\}
    
    \item \textit{Instruction replacement faults were shown to be possible in [B]. Can ARMORY evaluate such faults?}\\
    
        %\todo{Ja geht, beschrieben in...}\\
        \revise{
        Indeed \fsim is able to evaluate such faults out-of-the-box.
        We restructured our explanation in \Section{fsim::sec::armory::realworld}, paragraph ``Supported Fault Effects'', for better comprehensibility.
        }\\
    
    \item \textit{It would help to add a discussion on scalability. For example, bit-level faults offer many combinations on 32-bit devices, therefore the evaluation time is expected to grow high, in case of higher-order faults exponentially. A table/plot showing different code sizes (e.g. 100, 1000, 10000 instructions), w.r.t. evaluation time would help understand what is feasible.}\\
    
        %\todo{Tabelle/Figure?}\\
        \revise{
        We agree, simulation time is largely dependent on the number of injection points a specific model generates.
        However, estimating simulation time is not accurately possible from just this number, since the eventual effects of faults on the binary play a major role during simulation:
        invalid Assembly can be regarded as not exploitable immediately, while a change in a loop counter may result in several hundred more instruction executions before a decision on exploitability can be made.
        Hence, even if only 100 instructions would be faulted, simulation could still take longer than 1000 instructions, depending on the actual Assembly code and fault model.
        We added a dedicated remark to the end of \Section{fsim::sec::armory::strategy}.
        }\\
    
    \item \textit{In [C], it was shown that to evaluate encoding-based countermeasures, it is necessary to check all the possible values of a fault that can be injected as for a successful fault, it has to change the original codeword value to another. As most SIFA countermeasures are based on error detection codes, it is especially useful to check against such fault models. However, [C] only evaluates instruction-level faults. Would this type of analysis be feasible to do with ARMORY for both instruction and register faults?}\\
    
        %\todo{Ja, beliebige faults auf instruktionen und register möglich, geht zu evaluieren}\\
        \revise{
        Yes, this type of analysis is possible as \fsim supports arbitrary faults on instructions and registers.
        As we elaborate in \Section{fsim::sec::armory::realworld}, this combination is sufficient to cover a large set of real-world fault effects.
        }\\
    
    \item \textit{Section II.A: it would be good to elaborate more on different countermeasure techniques.}\\
    
        \revise{We added a thorough description of countermeasures against fault attacks, please see Sect. \ref{fsim::sec::background}.A.\\}
            
    \item \textit{Table 1: in register faults, what is the difference between "transient" and "until overwritten"?}\\
    
        %\todo{Steht im text du Affe}\\
        \revise{
        The different types of fault models were explained in \Section{fsim::sec::armory}.
        Regarding register faults, an until-overwrite fault affects a register value once but subsequent (over-)writes to the register will remove the fault's effect.
        This can be thought of on a high level as faulting the source of the register during load instructions. 
        Transient faults on registers are only valid for a single instruction execution after which the register returns to its unfaulted value.
        This can be compared to faulting the output bus of the register bank or faulting the operand buffers directly. 
        }
        
        \revise{
        We moved and improved these explanations into dedicated paragraphs for instruction and register fault models in our revised \Section{fsim::sec::armory::models}
        }\\
    
    
    \item[\text{[A]}] \textit{T. Given-Wilson, N. Jafri, J. Lanet and A. Legay, "An Automated Formal Process for Detecting Fault Injection Vulnerabilities in Binaries and Case Study on PRESENT," 2017 IEEE Trustcom/BigDataSE/ICESS, Sydney, NSW, 2017, pp. 293-300.}\\
    \item[\text{[B]}] \textit{S. V. Dilip Kumar et al., "A Practical Fault Attack on ARX-Like Ciphers with a Case Study on ChaCha20," 2017 Workshop on Fault Diagnosis and Tolerance in Cryptography (FDTC), Taipei, 2017, pp. 33-40.}\\
    \item[\text{[C]}] \textit{J. Breier, X. Hou and Y. Liu, "On Evaluating Fault Resilient Encoding Schemes in Software," in IEEE Transactions on Dependable and Secure Computing, 2019.}\\
    
    
\end{enumerate}

\thispagestyle{empty}
\subsubsection*{Reviewer 2}
\begin{enumerate}
    \item \textit{How is this simulator embedded in a design flow of IoT devices? It seems that fault models should be determined for each IoT device depending on the application of IoT devices because attack scenarios differ.}\\
    
        %\todo{see next}
        \revise{            
        This is correct.
        As in any kind of non-physical fault assessment, an analyst has to select suitable models for faults.
        In \fsim, all faults that were found to be exploitable are guaranteed to be correct by design as explained in Sections \ref{fsim::sec::armory::outputs} and \ref{fsim::sec::armory::realworld}.
        Hence, an analyst could also first apply \fsim with an overly powerful set of fault models, later filtering out those that were deemed to be infeasible.
        }
    
        \revise{
        With \Section{fsim::sec::armory::realworld} we added an entire section dedicated to \fsim in real-world applications, further discussing this issue.
        }\\
        
    \item \textit{This reviewer is not convinced with the explanation of ``exploitable fault” that appears in the manuscript many times. Similar to question 1, how do we set the rule of ``exploitable fault?”}\\
    
        %\todo{TODO Max: Armory in Real World Kapitel}\\
        \revise{
        We acknowledge that the notion of exploitability and according rules were scattered around the paper and improved this revision as follows.
        We introduce exploitability models in our Terminology Section \ref{fsim::sec::armory::terminology} and further detail on them when explaining the inputs to \fsim in our revised \Section{fsim::sec::armory::inputs}.
        In \Section{fsim::sec::armory::realworld} we further elaborate on the choice/selection an analyst must make in order to properly capture faults.
        Regarding our experiments, we precisely explain our exploitability model for each case study in the respective paragraphs of \Section{fsim::sec::casestudies}.
        Please also see our related answer to the next question.
        }\\
        
    \item \textit{Attackers’ ability to control faults is not discussed very well.
        I am afraid that this is due to the simple interface of ARMORY as for physical parameters. This reviewer understands RT-level is out of scope, but some attackers can access the layout information of the physical layout of ARM core. Please explain how ARMORY can change the configuration by the attack scenario?
        Also, please describe the cases where some noise occurs in injecting faults.}\\
    
        %\todo{RT-Level: out of scope, Erweiterung technisch möglich, aber aufwändig, eventuell in Future-Work Kapitel?}\\
        \revise{
        As the reviewer already noted, physical fault injection is not in the scope of this work.
        In fact, physical effects of faults are abstracted by the employed fault models, as common in works on fault assessment by simulation.
        This naturally neglects difficulties for an attacker such as noise during injection etc.
        In case RTL information is available to an analyst, this indeed is not supported in \fsim.
        While it would be technically possible to extend both \emu and \fsim to incorporate RTL information, this would be a tremendous effort and is primarily not intended.
        We briefly discuss this in the newly added \Section{fsim::sec::armory::realworld}.
        }\\
        
    \item \textit{Assessment of the output of ARMORY is not clear to this review. Could we perform a quantitative analysis using the simulation results of ARMORY? For instance, is the amount of leakage available with some post-processing of the results?}\\
        
        %\todo{Yes, output functions such as in Figure 3 is included in ARMORY.}\\
        \revise{
        Yes, outputs of \fsim can be used for a quantitative analysis, as they include precise information that suffices to reconstruct the fault.
        The results shown in \Figure{fsim::fig::experiment3} and \Figure{fsim::fig::experiment4} were also directly generated from the raw outputs of \fsim.
        However, note that a quantitative analysis has to be adjusted for the exploitability model.
        For instance, assume that any change to a specific register results in exploitable behavior. 
        Then, a single-bit fault model would result in much more exploitable faults than a byte-level fault model.
        We improved our presentation of \fsim's outputs in \Section{fsim::sec::armory::outputs}.
        }\\
        
\end{enumerate}

\thispagestyle{empty}
\subsubsection*{Reviewer 3}
\begin{enumerate}
    \item \textit{It is not very clear how the point of interests are chosen. Does ARMORY target every register and instruction in the sequence obtained from a fault-free simulation? Or it only targets a subset of them? Who decides the potential point-of-interests -- is it the user or the tool itself?}\\
        
        %\todo{Yes, exhaustively. “Point of injection” terminology section}\\
        \revise{
        The wording around ``point of interest'' was indeed misleading.
        \fsim works exhaustively, i.e., every register and every instruction is targeted, sometimes even multiple times.
        For example, a single-bit fault model is applied 32 times to a register.
        Hence there is no ``deciding'' what points are of interest for fault injection.
        Rather, faults are injected in every location that is accessed in a fault-free run.
        }
    
        \revise{
        Since the wording around ``point of interest'' was indeed misleading, we changed it to ``injection point'' and added a dedicated paragraph in our new terminology section \ref{fsim::sec::armory::terminology}.
        We also largely improved our explanation of how injection points are gathered in \Section{fsim::sec::armory::strategy}.
        }\\
        
        
    \item \textit{In Sec. V.B, authors assume that during higher-order fault simulation, if one fault model is found exploitable, then its combination with another fault model is also exploitable. This assumption also helps them to save simulation time. However, to me, this assumption seems optimistic. In reality, the information leakage created by one fault might get destroyed by another fault. Hence, it is not safe to conclude that if a fault model is exploitable, all its supersets are also exploitable.}\\
        
        %\todo{Yes fully agreed, but starting with low-order expl. Is more severe than higher order expl, => real world. Could be changed by user very easily if desired}\\
        \revise{
        Yes, we fully agree. 
        Another fault can oftentimes render the effect of the first fault useless, e.g., simply by crashing the chip due to invalid Assembly.
        However, our reasoning goes the other way around:
        an exploitable fault of lower order is much more severe than an exploitable fault of higher order due to the added complexity.
        Hence, we rather regard this early-exit as a severity-driven measure.
        In other words, invalidating the vulnerability by adding more faults does not fix the vulnerability at all, hence it is reasonable to report the least-effort-requiring vulnerability.
        }
    
        \revise{
        We improved our respective explanations in \Section{fsim::sec::armory::strategy}.
        }\\
        
    \item \textit{Page 5. line 59, 60, second column: "although several internal optimizations allow us to regard this as a very pessimistic." Please clearly state which are the optimizations that help you to reduce the complexity of higher-order fault simulations. Authors mentioned about multi-core support and M-ulator backups. However, these seem to be general tricks. No higher-order specific optimizations were found. Please concretely specify which optimizations you address in these lines.}\\
    
        %\todo{Ok rephrase}\\
        \revise{
        We agree that \Section{fsim::sec::armory::optimizations} discusses optimization strategies that, while being tailored to our fault simulation architecture, are not targeted specifically at higher-order simulation.
        }
    
        \revise{
        In light of our improved presentation regarding the previous question, which indeed is a dedicated optimization that benefits higher-order simulation, we slightly rephrased our introduction to \Section{fsim::sec::armory::optimizations}.
        }\\
        
    \item \textit{The authors use Tiny-AES for their case study. I would strongly suggest utilizing a full AES implementation.}\\
    
        \revise{
        The open-source \enquote{Tiny-AES} is indeed a full AES implementation.
        The (misleading) name originates from the target optimization: Tiny-AES is explicitly optimized for small embedded devices.
        }
    
        \revise{
        We improved our introduction of Tiny-AES in \Section{fsim::sec::casestudies::aes}.
        }\\
        
    \item \textit{The authors select a restricted set of fault models in their analysis. Classically, at least for cryptographic fault attacks, high-level fault models such as bit/byte/nibble faults are utilized. Even while processor-level faults are realized, their final impact culminates in one of such high-level fault model. For an exhaustive analysis tool, it is expected that it detects all possible valuations of (say) a byte fault at some specific location as exploitable. }\\
    
        %\todo{Yes indeed caused by the faulting tied to an instruction, (load/store)}\\
        \revise{
        There seems to be a slight misunderstanding of our fault models, which are actually not restricted as written by the reviewer.
        Simple fault models such as bit/byte/nibble faults are supported out-of-the-box.
        \fsim is able to detect all possible exploitable fault injections of these models.
        }
    
        \revise{
        We improved our explanation of fault models in \Section{fsim::sec::armory::models} for better comprehensibility and added a new \Section{fsim::sec::armory::realworld} which discusses implications of utilizing \fsim in real-world applications.
        }\\
        
    \textit{To better explain, let me consider the example of AES with single-byte fault injection. All 16 bytes at the beginning of 8th round are equally exploitable in this case. How can it be guaranteed that by the chosen low-level fault models, all such locations would be covered?}\\

        %\todo{Yes, exhaustively}\\
        \revise{
        This is guaranteed by the exhaustive nature of \fsim.
        By design, \textbf{all} points where the given fault model(s) can be applied are tested in simulation.
        Let us give an example of a byte-level register fault model:
        for every executed instruction \fsim scans the operands for registers and then applies the byte-fault model to each of the four bytes of the register, one after the other.
        After each injection, \fsim continues simulation to check whether the fault was exploitable.
        This way, the value of every utilized register is faulted on every possible byte on every instruction in the entire execution, i.e., simulation is exhaustive and does not miss a spot.
        }
        
    \item \textit{For deciding a fault as exploitable, authors use algorithm-specific tricks and only evaluated known threats. However, there exist generic algorithms for fault attack leakage assessment, such as in [1].}\\

        %\todo{Could be integrated as “evaluator”. However, only applicable to crypto (opposed to secure boot etc.)}\\
        \revise{
        Approaches such as [1] can simply be utilized as the exploitability model.
        Hence, a combination of approaches is not prohibited, but rather supported by \fsim.
        However, note that [1] is specifically designed for crypto, but fault attacks are also a threat to applications where the cryptographic elements are not a target, as in our secure bootloader case study.
        }\\
        
    \item[\text{[1]}] \textit{ALAFA: Automatic Leakage Assessment for Fault Attack Countermeasures. DAC 2019.}\\
        
    \end{enumerate}

\thispagestyle{empty}
\newpage
\setcounter{page}{1}
\twocolumn

